QDTrack: Quasi-Dense Similarity Learning for Appearance-Only Multiple Object Tracking

Similarity learning has been recognized as a crucial step for object tracking. However, existing multiple object tracking methods only use sparse ground truth matching as the training objective, while ignoring the majority of the informative regions in images. In this paper, we present Quasi-Dense Similarity Learning, which densely samples hundreds of object regions on a pair of images for contrastive learning. We combine this similarity learning with multiple existing object detectors to build Quasi-Dense Tracking (QDTrack), which does not require displacement regression or motion priors. We find that the resulting distinctive feature space admits a simple nearest neighbor search at inference time for object association. In addition, we show that our similarity learning scheme is not limited to video data, but can learn effective instance similarity even from static input, enabling a competitive tracking performance without training on videos or using tracking supervision. We conduct extensive experiments on a wide variety of popular MOT benchmarks. We find that, despite its simplicity, QDTrack rivals the performance of state-of-the-art tracking methods on all benchmarks and sets a new state-of-the-art on the large-scale BDD100K MOT benchmark, while introducing negligible computational overhead to the detector.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bib_photos/tobias-fischer.jpeg}}]{Tobias Fischer}
is a Ph.D. candidate in Computer Vision supervised by Prof. Dr. Fisher Yu at ETH Zurich, Switzerland. He obtained his M.Sc. and B.Sc. degrees in Computer Science from RWTH Aachen University, where he worked on 3D reconstruction and tracking at the Visual
Computing institute. His research interests lie in the area of 3D scene understanding, with a focus on retrieving 3D information from visual perception for object
recognition, tracking and reconstruction.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bib_photos/jiangmiao-pang.jpeg}}]{Jiangmiao Pang}
is a Research Scientist at Shanghai AI Laboratory. He obtained his Ph.D. degree from Zhejiang University and did his postdoc at MMLab, CUHK. He has worked with Dr. Jianping Shi at SenseTime, Prof. Fisher Yu and Prof. Trevor Darrell at UC Berkeley, and Prof. Dahua Lin at MMLab during his postgraduate study. His research is at the junction of machine learning, computer vision, and robotics. His long-term research goal is to build intelligent systems that can perceive and act like human beings.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bib_photos/thomas-huang.png}}]{Thomas E. Huang}
is a Ph.D. candidate in Computer Vision supervised by Prof. Dr. Fisher Yu at ETH Zurich, Switzerland. He obtained his M.S.E. and B.S.E. degrees in Computer Science from the University of Michigan, Ann Arbor in 2021 and 2019, respectively. His broad research interests are deep learning and its applications to computer vision. Recently, his research focuses on robust and sample-efficient learning, multi-object tracking, and multi-task learning.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bib_photos/linlu-qiu.png}}]{Linlu Qiu}
Linlu Qiu is a Ph.D. student at Massachusetts Institute of Technology. She obtained her M.S. degree from Georgia Institute of Technology and B.Eng. Degree from the University of Hong Kong. After that, she worked as an AI resident at Google Research.  Her recent research lies in the intersection of natural language processing and machine learning, with a focus on compositional generalization and grounded language understanding. 
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bib_photos/haofeng-chen.jpg}}]{Haofeng Chen}
Haofeng Chen received Master of Science in Computer Science in Stanford University, and Bachelor of Science in Computer Science in Georgia Institute of Technology. He worked in the Stanford Vision and Learning Lab on video understanding. Prior to Stanford, he worked at Berkeley DeepDrive on data annotation, 2D object detection, segmentation, and tracking.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bib_photos/trevor-darrell.jpeg}}]{Trevor Darrell}
is an Professor on the faculty of the CS and EE Divisions of the EECS Department at UC Berkeley. He founded and coleads Berkeley’s Berkeley Artificial Intelligence Research (BAIR) lab, the Berkeley DeepDrive (BDD) Industrial Consortia, and the recently launched BAIR Commons program in partnership with Facebook, Google, Microsoft, Amazon,
and other partners. He also is Faculty Director of the PATH research center at UC Berkeley, and previously led the Vision group at the UCaffiliated International Computer Science Institute in Berkeley. Prior to that, Prof. Darrell was on the faculty of the MIT EECS department from 1999-2008, where he directed the Vision Interface Group. He was a member of the research staff at Interval Research Corporation from 1996-1999, and received the S.M., and PhD. degrees from MIT in 1992 and 1996, respectively. He obtained the B.S.E. degree from the University of Pennsylvania in 1988.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bib_photos/fisher-yu.jpeg}}]{Fisher Yu}
is an Assistant Professor at ETH Zurich in Switzerland. He obtained his Ph.D. degree from Princeton University and became
a postdoctoral researcher at UC Berkeley afterwards. He directs the Visual Intelligence and Systems (VIS) Group. His research is
at the junction of machine learning, computer vision, and robotics.
\end{IEEEbiography}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
